Testing Neural Program Analyzers

Deep neural networks have been increasingly used in software engineering and program analysis tasks. They usually take a program and make some predictions about it, e.g., bug prediction. We call these models neural program analyzers. The reliability of neural programs can impact the reliability of the encompassing analyses. In this paper, we describe our ongoing efforts to develop effective techniques for testing neural programs. We discuss the challenges involved in developing such tools and our future plans. In our preliminary experiment on a neural model recently proposed in the literature, we found that the model is very brittle, and simple perturbations in the input can cause the model to make mistakes in its prediction.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
\begin{comment}
    In this paper, we proposed an approach for automatically generating synthetic test programs to verify the robustness of neural models. 
    We designed and implemented a set of different semantic transformations in programs for finding inconsistent behaviors in neural models. 
    We experimented \T{} on two state-of-the-art neural models and found that \T{} is successful in detecting erroneous behaviors of the neural models. 
\end{comment}

in this paper, we reported our ongoing project for testing neural programs.
and reported our ongoing attempts to 
uncover problem for those program 
